Which Strategies Matter for Noisy Label Classification? Insight into Loss and Uncertainty

Label noise is a critical factor that degrades the generalization performance of deep neural networks, thus leading to severe issues in real-world problems. Existing studies have employed strategies based on either loss or uncertainty to address noisy labels, and ironically some strategies contradict each other: emphasizing or discarding uncertain samples or concentrating on high or low loss samples. To elucidate how opposing strategies can enhance model performance and offer insights into training with noisy labels, we present analytical results on how loss and uncertainty values of samples change throughout the training process. From the in-depth analysis, we design a new robust training method that emphasizes clean and informative samples, while minimizing the influence of noise using both loss and uncertainty. We demonstrate the effectiveness of our method with extensive experiments on synthetic and real-world datasets for various deep learning models. The results show that our method significantly outperforms other state-of-the-art methods and can be used generally regardless of neural network architectures.

==> 03.related.tex <==
\section{Related Work}
% In recent years, a considerable amount of literature has been investigated to overcome corrupted labels by using prediction variance or loss. 

% \subsection{Variance-based approaches.}
Prediction variance is an indicator of how consistent the predictions are in a series of training and is often referred to as sample uncertainty~\cite{schein2007active}. Based on this prediction variance, two contradictory ideas have been developed.
% Two contradicting ideas have been developed based on prediction variance, which represents the uncertainty of samples~\cite{schein2007active}. 
Prioritizing samples with high prediction variance is one approach. For example, \textit{Decoupling}~\cite{malach2017decoupling} consists of two neural networks and updates networks only with instances that predict inconsistently, thus emphasizing high variance samples. Likewise, \textit{Active Bias}~\cite{chang2017active}, a method impervious to the difficulty of tasks, focuses on uncertain samples by using the history of previous prediction probabilities. In contrast to methods that emphasize samples with high variance, some methods take the opposite approach. An example is \textit{SELFIE}~\cite{song2019selfie}, which removes samples with high variance while correcting the labels of samples with consistent predictions.
 
 
% \subsection{Loss-based approaches.}
Loss can signify the difficulty and the confidence of predictions, so giving precedence to samples with low loss or those with high loss can work well depending on the amount of noise in the data or the complexity of the problem~\cite{hinton2007recognize,loshchilov2015online}. One line of approaches emphasize difficult samples. \textit{Hard example mining}~\cite{shrivastava2016training}, for example, takes advantage of hard samples and eliminates easy samples which comprise a large part of the training data, resulting in improved training convergence. Although difficult samples can accelerate training in some cases~\cite{malisiewicz2011ensemble}, Chang et al.~\cite{chang2017active} showed that easy samples are effective when solving a challenging task such as training with severe label noise. As a result, recent research has focused on easy samples based on loss. An example is \textit{MentorNet}~\cite{jiang2017mentornet}. A pretrained mentor network provides a sample weighting scheme for the student network to emphasize easier samples which are likely to be correct. Similarly, \textit{Co-teaching}~\cite{han2018co} obtains better performance by simultaneously training two networks on easy samples selected by one another. Some methods also adopt a similar approach by using samples with low loss as training data and filtering out samples with high loss values~\cite{huang2019o2u, chen2019understanding, song2019selfie}. We adopt a similar approach as those that select easy samples for training, for it is known that removing noisy data and training with a cleaner subset is generally better~\cite{frenay2013classification}. However, we present a refined version which does not require additional networks, unlike prior studies.

To the best of our knowledge, there remains an unresolved question whether it is beneficial to increase or decrease the importance of samples based on variance and loss. In this paper, we seek to determine which strategy is most efficacious for robust training with noisy labels. Based on such findings, we propose a novel and simple method \prgname{}, and empirically validate its performance.




==> 10.broader_impact.tex <==
\section{Broader Impact}

Deep learning models have been of great interest for many years due to its critical impact on the economy and its integral role in guiding individuals, companies and organizations to automate processes and make informed decisions. Deep learning requires numerous amounts of data, so there is a high demand of data collection which entails crawling data from the web or labeling by workers. However, such collection of data naturally includes label noise, and these noisy data can severely deteriorate model performance even though they are collected to improve performance. As a result, robustly training models with label noise have generated considerable recent research interest. In particular, many researchers have enhanced performance using uncertainty and loss but have ironically employed contrasting strategies. To elucidate how contradicting approaches can improve learning with label noise, we have analyzed in depth how loss and uncertainty appear differently in noisy samples compared to clean samples, and propose a new method based on these insights. Through rigorous experiments, we have shown that our method performs well on data with various types and conditions of noise, thus satisfying the realistic desire for a promising strategy. Our method, therefore, has a great impact on society because it can be easily applied and guarantees high performance regardless of model architectures and without any additional clean data.

Because large amounts of data are required to increase accuracies of deep learning models, crawling data from the web and labeling data manually have become popular ways to collect data. Both approaches, however, may have negative societal impacts. First, using data from the web can cause ethical dilemmas such as invasion of privacy. We, therefore, have used datasets that have been publicly released and have confirmed not to redistribute the Clothing1M dataset and only use the data for academic purposes. Second, although developing methods that learn from data with noisy labels can relieve the workload of labelers, there nevertheless runs the risk of potential job loss that could occur due to the decreasing need of labeling workers. In our setting, more labeled data can be a remarkable way of increasing model performance, so the demand of workers still remains. Furthermore, labelers can benefit using our method because their mistakes become insignificant.



==> tab-data.tex <==
\setlength{\tabcolsep}{5pt}
\ctable[
% 	captionskip = -2pt,
    caption = {Details of datasets used in the experiments.},
    label = tab:data,
%    pos=tbp,
%    width=tabularx,
%    figure,
%    star,
%       doinside=\small
     doinside = \footnotesize
%     doinside = \scriptsize
   % doinside = \tiny
]{ccccc}{
\tnote[$\ast$] {a subset of ImageNet~\cite{deng2009imagenet} \wy{++  TODO: shorten this gap ++ }}
}{
\toprule
 Dataset & Train \# & Test \# & Class \# & Image size \\
\midrule
CIFAR-10            & 50K                 & 10K                & 10            & 32x32      \\ 
CIFAR-100           & 50K                 & 10K                & 100           & 32x32      \\ 
Tiny ImageNet$^\ast$     & 100K                & 10K                & 200           & 64x64      \\ 
Clothing1M     & 1M noisy                & 10K                & 14           & 256x256      \\ 
\bottomrule
}
